The Programmable Data Plane: Abstractions, Architectures, Algorithms, and Applications

Programmable data plane technology enables the systematic reconfiguration of the low-level processing steps applied to network packets and is a key driver in realizing the next generation of network services and applications. This survey presents recent trends and issues in the design and implementation of programmable network devices, focusing on prominent architectures, abstractions, algorithms, and applications proposed, debated, and realized over the past years. We elaborate on the trends that led to the emergence of this technology and highlight the most important pointers from the literature, casting different taxonomies for the field and identifying avenues for future research.

==> txt/hardware.tex <==
When reasoning about the factors that brought programmable data plane solutions to a quick industrial adoption, many agree that the compatibility of early abstractions with legacy switching hardware was a key element~\cite{roadtosdn}. As such, many of the design decisions, programming abstractions, and envisioned applications are better explained when starting with an understanding of the hardware platforms used for the implementation of a network data plane.

The rest of this section provides an overview on the matter, describing the three main types of platforms: application-specific hardware, i.e., ASICs; System-on-Chip (SoC) solutions, e.g., Network Processors; general purpose systems, e.g., commodity server machines.
Before diving in the details of such architecture, next we provide a brief primer on the operations performed during packet processing.

\subsection{Packet Processing}
Packet processing entails five logic steps: \textit{parsing}, \textit{classification}, \textit{modification}, \textit{deparsing}, \textit{forwarding}.

\textit{Parsing} is the process of locating the packet header in the data, and extracting its fields' values. Such values are then used during \textit{classification}, i.e., the process that matches a given packet with the corresponding forwarding policy, in order to identify the right forwarding decision for the packet, e.g., which output port to use, as well as the required packet modification actions, e.g., rewriting a header's filed. The \textit{modification} step applies the actions retrieved during classification, and may include also the collection of statistics related to the packet processing, e.g., to increase flow's counters. Once all the modifications are applied, the \textit{deparsing} step assembles a new packet, which includes the modified packet headers, as well as the original packet body. Finally, \textit{forwarding} is the step of sending the assembled packet to an output port for trasmission. This step may include the implementation of scheduling policies, e.g., for the implementation of Quality of Service (QoS) guarantees.


\subsection{Switching ASICs}
A switching ASIC is specialized in performing packet processing, focusing on implementing just the set of operations required for such task. In fact, network devices built using ASICs generally include a second general purpose sub-system, e.g., based on CPUs, in order to implement the device's monitoring and control functions, as well as more complex (and uncommon) packet processing functions that the ASIC does not support. The processing in ASIC is usually called the \textit{fast path}, by contrast, the \textit{slow path} is the processing done by the general purpose sub-system.

A typical ASIC design is organized as a fixed pipeline of stages that performs sequentially the packet processing steps, as outlined earlier.
When a packet is received, the packet parser extracts the values of the packet header's fields, and stores them in a so-called \textit{metadata} bus, which can be accessed throughout the processing pipeline. In many cases, the metadata bus is limited to a size of few hundreds bytes~\cite{bosshart:rmt}, which also limits the number and size of values that can be parsed.  The packet body is instead stored in a separated packet buffer, which is accessed only after a packet forwarding decision has been taken, in order to copy the data to the destination output port.

The values stored in the metadata bus are used for the classification step, which is implemented using lookup tables. Such tables can be both organized as a sequential pipeline, or sometime they may operate also in parallel, to reduce processing latency. Each table is specialized (or programmed) to match on a subset of the extracted header fields. The tables may further have different matching capabilities depending on the way they are implemented by the hardware. For instance, exact matching tables could be implemented as hashtables in an SRAM, while wildcard matching tables are generally implemented using more expensive TCAM.

The outcome of the classification step provides the packet modification instructions that are applied in the last processing step. Fast arrays of Arithmetic Logic Units (ALUs) are employed to implement such instructions in parallel on the data contained in the metadata bus. Since such bus also contains the information about the destination output port of the packet, potentially including information relevant for priority and scheduling decisions, modifying such values actually corresponds to the definition of the packet's forwarding action.

The data in the metadata bus are finally used by the deparser to reassemble the packet, before passing it to the forwarding step, along with the priority and scheduling information. Finally, the packet is generally handled by a scheduler block that transmits it to the designed output port.

The above structure may be repeated, more than once in a switching ASIC. For instance, it is common to have multiple classification and modification stages between the parsing and deparsing steps. Furthermore, in many switches it is common to have at least two such pipelines, generally named the ingress and egress pipeline.

\subsection{Network Processors}
SmartNICs have an architecture that comprises several different hardware blocks. Some blocks are dedicated to network-specific operations that have to do with e.g., load balancing, encryption, etc. Some other hardware resources are instead dedicated to programmable components that are generally used to implement new network protocols and/or packet operations. The Netronome NFP programmable architecture is shown in Fig.~\ref{fig:netronome} and described next.

Since network traffic is a mainly parallel workload, with packets belonging to independent network flows, these devices are optimized to perform parallel computations, with several processing cores. In Netronome terminology, a programmable processing core is named micro-engine (ME). The programming of MEs happens, among other means, using a C dialect called \textit{micro-C}. The language is essentially a version of C extended with constructs and functions that are specific to the NFP chip.
Each ME has 8 threads, which share local registries that amount for a total of 4KB. MEs are further organized in islands, and each island has two shared SRAM memory areas of 64KB and 256KB, called CLS and CTM, respectively. Generally, these memory areas are used to host data required for the processing of each network packet. Finally, the chip provides a memory area shared by all islands, the IMEM, of 4MB SRAM, and a memory subsystem that combines two 3MB SRAMs, used as cache, with larger DRAMs, called EMEMs. These larger memories generally host the forwarding tables and access control lists used by the networking subsystem to decide how to forward (or drop) a network packet.
MEs can communicate and synchronize with any other ME, irrespective of the location (i.e., same or different islands). Of course, communications across islands take longer and may impact the performance of a running program.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\columnwidth]{imgs/nfp.png}
    \vskip -10pt
    \setlength{\belowcaptionskip}{-15pt}
% Taken from https://p4.org/assets/p4_d2_2017_nfp_architecture.pdf
    \caption{The architecture of a Netronome NFP4000's programmable blocks. Other hardware blocks specialized for network packet processing are not shown.}
    \label{fig:netronome}
    \vspace{-1.5em}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

